Output-feedback adaptive model predictive control for ramp metering: a set-membership approach

Ramp metering, which regulates the flow entering the freeway, is one of the most effective freeway traffic control methods. This paper introduces an output-feedback adaptive approach to ramp metering that combines model predictive control (MPC) with set-membership parameter and state estimation. The set-membership estimator is based on a mixed-monotone embedding of underlying traffic dynamics. The embedding is also used as the modeling basis for MPC optimization. For a freeway stretch with unknown parameters and partial measurement on the freeway mainline, we provide sufficient conditions on the control horizon, cost functions, terminal sets of MPC, and inflow demand at the ramps such that the queue lengths in the closed-loop system remain bounded. The sufficient condition on the demand matches the necessary condition, thereby proving maximal throughput under the proposed controller. The result is strengthened to input-to-state stability when model parameters and demand are known. The stability analysis is conducted for the case of constant demand and unbounded on-ramps. The closed-loop trajectory data generated by the proposed controller is shown to facilitate finite time estimation of free-flow model parameters, i.e., free-flow speed and turning ratios. Simulation results illustrate stability of the closed-loop system under the proposed controller with time-varying demand and few mainline measurements, for which the system becomes unstable under a well-known approach from the literature. This indicates that the proposed controller renders higher throughput than the well-known approach, possibly using more computing resources.

==> Gas-MPC-zl.tex <==
\section{Control of gas pipeline}

Consider a gas pipeline partitioned into $I$ cells with length $\Delta L$, cross-section diameter $D$ and area $A$. Let $p_i(t)$ and $q_i(t)$ be the pressure and outflow rate of the $i$-th cell at time $t$. Let $u(t)$ denote the incoming flow rate at the begining of the pipeline that is assumed to be controlled. Let $\lambda$ denote the required outflow rate at the end of the pipeline that is determined exogenously. We use the following dynamics for the gas pipeline by spatially and temporally discretizing the a PDE model, see \cite{gugat2020closed} :
\begin{equation}\label{eq:gas-dynamics}
	\begin{aligned}
		&p_1(t+1) =p_1(t) + c^2\dfrac{\Delta T}{\Delta L}\left(u_0(t) - q_i(p(t))\right), i\in[I] \\
		&q_i(p(t))=\text{sgn}\left(p_i(t) - p_{i+1}(t)\right)\\ & \hspace{.65in}\sqrt{\dfrac{2DA}{c^2\mu\Delta L}p_i(t)\lvert p_i(t) - p_{i+1}(t)\rvert}, i\in[I-1] \\
		&q_I(p(t)) = \lambda
	\end{aligned}
\end{equation}
where $\text{sgn}(\cdot)$ is the sign function; $c$ represents the speed of sound and $\mu$ represents friction coefficient. Let $p(t):=[p_1(t),p_2(t),\ldots,p_I(t)]$ be the state of the model, and the state space is $\mc P:=[0,\infty)^I$. For measurement information, we consider the following output:
\begin{equation}\label{eq:gas-output}
	y(t) = \mathbf{C}\, p(t)
\end{equation}
for appropriate, not necessarily invertible matrix $\mathbf{C}$.
\begin{example}
	There are pressure gauges installed at different locations of gas piplines that give pressure measurements \cite{sundar2018state}. Therefore, if a subset of cells are installed with pressure gauges, $\mathbf{C}$ in \eqref{eq:gas-output} is a diagonal matrix, with zero diagonal entries corresponding to missing gauges on the corresponding cells.
\end{example}

 In principle, there is no upper bound on the state in the model \eqref{eq:gas-dynamics}. However, in reality there are engineering limits on the pressure of gas piplines for the purpose of safey. Also, there are minimum requirements on the pressure of deliverable gas flow, i.e., \begin{equation}\label{eq:gas-pressure-constraint}
 	p^{\min}_i\leq p_i(t)\leq p^{\max}_i, \forall i\in[I], \forall t\geq0.
 \end{equation}
 
 We assume the incoming flow is nonnegative and upper bounded, and therefore $u(t)$ satisfies:
 \begin{equation}\label{eq:gas-u-constraint}
 	0\leq u_0(t)\leq u_0^{\max},\forall t\geq0
 \end{equation}
 
Our goal is to design a control signal $\{u_0(t):t\geq0\}$ that minimizes the cost of control $\sum_{t=0}^{\infty} u_0(t)$ subject to \eqref{eq:gas-dynamics}-\eqref{eq:gas-u-constraint} for a given non-negative coefficient vector $l$. Similar to \eqref{eq:finite-horizon-cost}, we use the MPC that recursively solves a related finite horizon problem at every time $t$:
   \begin{equation}
   	\label{eq:gas-finite-horizon-cost}
   	\sum_{s=t}^{t+T-1} u_0(s)
   \end{equation}
subject to \eqref{eq:gas-dynamics}-\eqref{eq:gas-u-constraint}.

In analogue to the MPC controller for ramp metering in \Cref{sec:mpc-set-membership}, we first modify the flow function by incorporating an auxiliary state $\nu$ as follows:
\begin{equation}
		\tilde{q}_i(p,\nu) =  \text{sgn}(p_{i}^2 - \nu_{i} \nu_{i+1})
		\sqrt{\dfrac{2DA}{c^2\mu\Delta L}\lvert p_{i}^2 - \nu_{i}\nu_{i+1}}\rvert,\forall i\in[I]
\end{equation} Then, we construct a decomposition function for gas dynamics as follows:
\begin{equation}
	\begin{aligned}
			F^{\text{gas}}_1(p,\nu,u_0) &= p_1(k\mid t) + c^2\dfrac{\Delta T}{\Delta L}\left(u_0- q_1(p)\right) \\
			F^{\text{gas}}_i(p,\nu,u_0)  &= 
			\begin{cases}
			p_i + c^2\dfrac{\Delta T}{\Delta L}\left(\tilde{q}_{i-1}(p,\nu) - q_i(p)\right)\text{ if }p_{i-1}\leq \dfrac{p_i}{2} \\
			p_i + c^2\dfrac{\Delta T}{\Delta L}\left(q_{i-1}(p) - q_i(p)\right)\text{ if }p_{i-1} > \dfrac{p_i}{2}
				\end{cases} \\ &\hspace{2.1in} i\in[2:I]
	\end{aligned}
\end{equation}

Given $\hat{p}(t), \hat{\nu}(t)\in\mc P$ as initial conditions, let $\mathrm{P}^{\text{gas}}(\hat{x}^m(t), \hat{\nu}^m(t))$ denote the following MPC optimization problem
\begin{equation}\label{eq:gas-mpc-opt}
	\begin{aligned}
		&\minimize_{\substack{\hat{u}_0(0:T-1\mid t)}} \quad \sum_{k=0}^{T-1}\hat{u}_0(k\mid t) \\
		&\subjecto\\
		& p(k+1\mid t) = F^{\text{gas}}(p(k\mid t),\nu(k\mid t), \hat{u}_0(k\mid t)), k \in[0,T-1]\\
		& \nu(k+1\mid t) = F^{\text{gas}}(\nu(k\mid t),p(k\mid t), \hat{u}_0(k\mid t)), k \in[0,T-1]\\
		&p(k\mid t), \nu(k\mid t) \text{ satisfies \eqref{eq:gas-pressure-constraint}}, \hat{u}_0(k\mid t)\text{ satisfies \eqref{eq:gas-u-constraint}}, \\ &\hspace{2.1in} \forall \, k\in[0:T-1] \\
		&p^m(0\mid t) = \hat{p}^m(t), \nu^m(0\mid t) = \hat{\nu}^m(t)
	\end{aligned}
\end{equation}

Under \Cref{ass:C-matrix}, the MPC-set membership method for the gas pipeline is described as follows: 
\begin{equation}\label{eq:gas-mpc-estimation}
	\begin{aligned}
		&\text{Initialize } \bar{p}(0),\ubar{p}(0). \\
		&\text{Update: } \forall i\in[I],\forall t\geq0 \\
		&\hat{\bar{p}}(t) = \left\{
		\begin{aligned}
			&\dfrac{y_i(t)}{c_{i,i}},\ c_{i,i}\neq 0 \\
			&\bar{p}_i(t),\ \text{o.w.}
		\end{aligned} \right.,
		\hat{\ubar{p}}_i(t) = \left\{
		\begin{aligned}
			&\dfrac{y_i(t)}{c_{i,i}},\ c_{i,i}\neq 0 \\
			&\ubar{p}_i(t), \ \text{o.w.}
		\end{aligned} \right. \\
		&\text{MPC: Solve $\mathrm{P}^{\text{gas}}(\hat{\bar{p}}(t), \hat{\ubar{p}}(t))$ in \eqref{eq:mpc-opt} to obtain $u_0(t)$}. \\
		&\text{Predict:} \\
		&\begin{aligned}
			\bar{p}(t+1) &= F(\hat{\bar{p}}(t), \hat{\ubar{p}}(t), u_0(t))\\
			\ubar{p}(t+1) &= F(\hat{\ubar{p}}(t), \hat{\bar{p}}(t), u_0(t)). \\
		\end{aligned}
	\end{aligned}
\end{equation}

==> MPC-MHE-computation-ks.tex <==
\section{Computational Considerations for the MPC-MHE Ramp Metering Controller}
\label{sec:computation}

The maximal element in $\mc X^m$ can be found by solving an LP, as follows. Consider an auxiliary state $x^a(s):=f_I(x^m(s-1))$. The dynamics of the augmented state is then: 
\begin{equation}\label{eq:cell-augmented-dynamics}
\begin{aligned}
		\begin{bmatrix}x_1^m(s+1)\\ x_2^m(s+1)\\ x_3^m(s+1)\\ \vdots \\ x_I^m(s+1)\\ x^{a}(s+1))\end{bmatrix} = \begin{bmatrix}x_1^m(s)\\ x_2^m(s)\\ x_3^m(s)\\ \vdots \\ x_I^m(s)\\0\end{bmatrix}+ \underbrace{\begin{bmatrix}
1 & -1 & 0 & \ldots & 0 & 0 \\
0 & \beta_1 & -1 & \ldots & 0 & 0 \\
0 & 0 & \beta_2 & \ldots & 0 & 0 \\
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
0 & 0 & 0 & \ldots & \beta_{I-1} & -1\\
0 & 0 & 0 & \ldots & 0 & \beta_{I}
\end{bmatrix}}_{\tilde{\mathbf{R}}} \tilde{f}(s) + \begin{bmatrix}u_1(s) \\ u_2(s) \\ u_3(s) \\ \vdots \\ u_I(s) \\ 0
\end{bmatrix}\\
	\end{aligned}
	\end{equation}
where 
\begin{equation}
\label{eq:flow-augmented}
\tilde{f}(s)=[0 \, \, \, f_1(x^m(s)) \, \, \, f_2(x^m(s)) \, \, \, \ldots \, \, \, f_{I-1}(x^m(s)) \, \, \, f_I(x^m(s))]^{\top}
\end{equation}
%\begin{equation*}
%\tilde{f}(x^m,u):= 
%\begin{bmatrix}
%0 \\ f_1(x^m) \\ f_2(x^m) \\ \vdots \\ f_{I-1}(x^m) \\ f_I(x^m)
%\end{bmatrix}, \quad
%\tilde{\mathbf{R}} :=
%\begin{bmatrix}
%0 & -1 & 0 & \ldots & 0 & 0 \\
%0 & \beta_1 & -1 & \ldots & 0 & 0 \\
%0 & 0 & \beta_2 & \ldots & 0 & 0 \\
%\vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
%0 & 0 & 0 & \ldots & \beta_{I-1} & -1\\
%0 & 0 & 0 & \ldots & 0 & \beta_{I}
%\end{bmatrix}, \quad
%\tilde{u}:=\begin{bmatrix}u_1 \\ u_2 \\ u_3 \\ \vdots \\ u_I \\ 0
%\end{bmatrix}
%\end{equation*}
%Let $\tilde{f}_1(x^{m}(t),u(t)) := u_1(t),\ \tilde{f}_{i+1}(x^{m}(t),u(t)):=f_i(x^m(t))\ i\in[I];\ \beta_0=1,\ \tilde{\mathbf{R}}:=\text{diag}(\beta_{i}, i\in\{0,\ldots,I\}), \mathbf{J}:=[j_{i,i+1} = 1; j_{i,k} = 0\ \forall k\neq i+1;i\in[I] ], \tilde{u}(t):=\begin{bmatrix}0 \\ u_i(t)\ i\in\{2,\ldots,I\} \\0
%\end{bmatrix}$
%

\begin{proposition}\label{prop:maximal-element-LP}
	Given applied input sequence $u(t-L:t-1)$ and measured output sequence $y(t-L:t)$, the maximal element $\hat{x}^{\circ,m}\in\mc X^m$ corresponds to the unique optimal solution to the following optimization problem:
	\begin{equation}
	\label{eq:lp-maximal}
\begin{split}
			&\underset{\substack{x^m(t-L:t), x^{a}(t-L:t)\\ u(t-L:t-1), \tilde{f}(t-L:t-1)}}{\text{maximize}}\ \mathbbm{1}^\top \tilde{\mathbf{R}}^{-1}\begin{bmatrix}x^m(t)\\x^a(t)\end{bmatrix} \\
	 \text{s.t.} & \, \,	\eqref{eq:cell-augmented-dynamics}, \quad s \in [t-L:t-1] \\
			&\tilde{f}_1(s) = u_1(s), \, \tilde{f}_{i+1}(s) \leq f_i(x^m(s)),\, i\in[I], \quad s \in [t-L:t-1] \\
			&y^m(s) = \mathbf{C}\ \! x^m(s), \quad \ s\in [t-L:t] \\
			&0\leq x^m(t-L) \leq \bar{x} \\	
		\end{split}
		\end{equation}
%		\begin{align}
%		\nonumber	&\underset{\substack{x^m(t-L:t), x^{a,m}_{I+1}(t-L:t)\\\tilde{u}(t-L:t-1), \tilde{f}(t-L:t-1)}}{\text{maximize}}\ \mathbbm{1}^\top(\tilde{\mathbf{R}}-\mathbf{J})^{-1}\begin{bmatrix}x^m(t)\\x^{a,m}_{I+1}(t)\end{bmatrix} \\
%	 s.t.\ &	\begin{bmatrix}x^m(s+1)\\x^{a,m}_{I+1}(s+1))\end{bmatrix}  = \begin{bmatrix}x^m(s)\\0\end{bmatrix}+ (\tilde{\mathbf{R}}-\mathbf{J})\tilde{f}(s) + \tilde{u}(s)			\label{eq:constraint-augmented-dynamics} \\
%		\nonumber	&\tilde{f}_1(s) = u_1(s) \\
%							   &	\tilde{f}_{i+1}(s) \leq f_i(x^m(t)) \text{ defined in }\eqref{eq:cell_dynamics},\ i\in[I] \label{eq:constraint-augmented-flow} \\
%		\nonumber	&\tilde{u}_1(s) = 0, \tilde{u}_{i+1}(s) = u_{i+1}(s), i\in[I-1],\ \tilde{u}_{I+1} = 0\\
%		\nonumber	&y^m(s) = \mathbf{C}\ \! x^m(s) , \text{for all}\ s\in\{t-L,\ldots,t-1\} \\
%		\nonumber	&0\leq x^m(t-L) \leq \bar{x} \\
%		\end{align}
\end{proposition}
%\begin{proof}
%	The proof of Proposition~\ref{prop:maximal-element-LP} is given in Appendix~\ref{proof:maximal-element-LP}
%\end{proof}

One can utilize Proposition~\ref{prop:maximal-element-LP} to show that \eqref{eq:saddle_point} can be equivalently written as a MILP. However, this may not be desirable for computational reasons. One can address this if (i) the outflows from the on-ramps can always be accommodated by the mainline, namely the second constraint in \ref{eq:u-constraint} is assumed to hold at all times and the flow function is modified to $f_i(x^m(t))= \min\big\{v_ix^m_i(t),\frac{w_{i+1}}{\beta_{i}} \big(\bar{x}^m_{i+1}-x^m_{i+1}(t)		-u_{i+1}(t)\big), \Cm_i\big\}, \, i \in [I-1]$; 
(ii) the terminal constraint $x(t+T)\in\mc X_f$ holds for sufficiently large $T$; and (iii) $l^{m\top}(\IR)$ and $b^{m\top}(\IR)$ are non-negative. Assumptions (i) and (ii) are common, e.g., see \cite{GOMES2006244,schmitt2018exact}. \kscomment{Indeed, \cite{grune2012nmpc} claims that (ii) not be necessary for stability for sufficiently large $T$.} \ksmargin{need exact reference if possible} If the three assumptions hold true, then \eqref{eq:saddle_point} can be shown to be equivalent to the following linear program: \ksmargin{include missing range of $s$}
	\begin{equation}\label{eq:min-LP}
		\begin{aligned}
			&\underset{\substack{x(t-L:t+T), u(t:t+T-1) \\f(t-L:t+T-1)}}{\text{minimize}}%_{\substack{u(t:t+T-1) \in \mc U}} %_{\hat{u}(t:t+T-1)\in\mathcal{U}}
			\sum_{s=t}^{t+T-1}l^\top  \, x(s)+ b^\top \, x(t+T) \\
			\text{s.t.} \ &(\IR)^{-1}x^m(s+1) = (\IR)^{-1}x^m(s) -f(s) + (\IR)^{-1}u(s) \\
			%\text{s.t. }\, x^m_i(s+1) &= x^m_i(s) + \beta_{i-1}f_{i-1}(s) - f_{i}(s)+ u_{i}(s),
			&x^r_i(s+1) = x^r_i(s) - u_{i}(s) + \lambda_i,\ i \in [I],\ \\
			&f_i(s) \leq \min\left\{v_{i}x^m_{i}(s), \frac{w_{i+1}}{\beta_{i}} \big(\bar{x}_{i+1}-x^m_{i+1}(s)-u_{i+1}(t)\big), \Cm_i\right\}, i\in [I-1]\,  s\in[t-L:t+T-1]\\
			&f_{I}(s) \leq \min\{v_I x^m_I(s),\Cm_I\},  \,  s\in[t-L:t+T-1] \\
			&x(t-L) = \begin{bmatrix} \hat{x}^{\circ,m} \\ x^r(t-L) \end{bmatrix} \\
			&u_i(s)\in[0,\min\{\bar{u}_i,x_i^{r}(s) +\lambda_i\}], \, i\in [I],\, s \in [t:t+T-1] 
		\end{aligned}
		\end{equation}
%in the sense that the optimal values of the minimization in \eqref{eq:saddle_point} and \eqref{eq:min-LP} are equal, and every optimal solution $u^*(t:t+T-1)$ to \eqref{eq:min-LP} is an optimal solution to the minimization in \eqref{eq:saddle_point}.


==> MPC-adaptive-stability-zl.tex <==
\section{Properties of the output-feedback MPC controller}
\label{sec:stability-adaptive-mpc}
First, we analyze the feasibility of the optimization \eqref{eq:mpc-opt}. In this study, we consider terminal sets to be box constraints, i.e., $\mc X_f := \{x:0\leq x^m\leq \xterm\}, \mc Z_f := \{z^m:0\leq z^m\leq \xterm\}$ where $\xterm\geq 0$ are user-defined parameters. In other words, we want the terminal mainline state to be bounded above by $\xterm$ and the queue length of on-ramps to be bounded above by $\xterr$. 
\begin{proposition}
	\label{prop:feasible-control-adative}
	Let inflow $\lambda$ satisfy \eqref{eq:max-flow} with strict inequalities. Then, for every $x^m,z^m\in\mc X^m, x^r\in\mc X^r$, and $\xterm\geq x^{\text{up}},\xterr\geq0$, $\mathrm{P}(x^m,z^m,x^r)$ is feasible for sufficiently large $T$.
\end{proposition}	
%\begin{remark}
%    The proof of \Cref{prop:feasible-control-non-empty} gives an explicit control policy which \eqref{eq:mpc-opt}. To derive a lower bound of $T$ for certain demand $\lambda$, initial conditions $\hat{x}(t), \zlbm(t)$, and upper bounds $\bar{x}^m$ and $\bar{x}^r$, one can apply the control \eqref{eq:vanishing-queue-policy} and simulate the dynamics for $T_{\text{lb}}$ steps until $x(T_{\text{lb}}\mid t)\in\mc X_f$. We denote such a lower bound as $T_{\text{lb}}\left(\hat{x}(t), \zlbm(t),\lambda,\bar{x}^m,\{x}^r\right)$.
%\end{remark}

Now we find sufficient conditions under which the closed-loop system consisting of \eqref{eq:cell_compact_dynamic}, \eqref{eq:output_measurements} in feedback with the MPC-set membership controller in \eqref{eq:estimation} is \emph{input-to-state  stable}. In this context, the exogenous inflow $\lambda$ is interpreted as the \emph{input}. In addition to \Cref{ass:C-matrix} and feasibility conditions in \Cref{prop:feasible-control-non-empty}, the sufficient conditions are on the terminal sets and the cost coefficients but not on number of cells with available measurements. Let $b := \begin{bmatrix} b^m \\ b^r \end{bmatrix}$ where $b^m$ and $b^r$ denote the cost coefficients for the mainline and on-ramps respectively:	

\begin{theorem}\label{theo:ISpS}
	Let \Cref{ass:C-matrix} hold.
	Let the inflow $\lambda$ satisfy \eqref{eq:max-flow} strictly and $T$ be sufficiently large such that $\mathrm{P}(\xupm(0),\zlbm(0),y^r(0))$ is feasible. Suppose there exists a control $u$ satisfying \eqref{eq:u-constraint} such that 
	\begin{equation}\label{eq:terminal-lyapunov}
		\begin{aligned}
			&b^\top\begin{bmatrix}
				F(x^m,z^m,u) \\ x^r - u + \lambda
			\end{bmatrix} - b^\top x \leq -l^\top x+b^{m\top}\lambda \\
			& \begin{bmatrix}
				F(x^m,z^m,u) \\ x^r - u + \lambda
			\end{bmatrix}\in\mc X_f, F(z^m,x^m,u)\in\mc Z_f, \\ & 
			\hspace{1.2in}\quad \forall \, x\in\mc X_f, z^m\in\mc Z_f.
		\end{aligned}
	\end{equation}
	Then, the following holds:
	\begin{enumerate}[leftmargin=0pt,itemindent=2em]
		\item (\emph{Recursive feasibility}) $\mathrm{P}(\xupm(t),\zlbm(t),y^r(t))$ in \eqref{eq:estimation} is feasible for all $t\geq0$. \label{result:recursive-feasibility}
	\item  (\emph{Input-to-state stability}) \label{result:ISS} 
	The closed-loop system consisting of \eqref{eq:cell_compact_dynamic}, \eqref{eq:output_measurements} in feedback with the output-feedback MPC controller in \eqref{eq:mpc-opt} is \emph{input-to-state  stable} with respect to $\lambda$, i.e.,
	\begin{equation}\label{eq:ISS-bound}
		\begin{aligned}
	     &\lVert x(t)\rVert_1 \leq \dfrac{\tilde{a}_2}{\tilde{a}_1} \rho^{t}\lVert \xupm(0) + y^r(0)\rVert_1 + \dfrac{\tilde{a}_3 + 2(1-\rho)\tilde{a}_2}{\tilde{a}_1(1-\rho)}\lVert \lambda \rVert_1,\\
	     &\hspace{2.1in} \forall\, t\geq 0,\quad \forall\, x(0)\in\mc X
		\end{aligned}
	\end{equation}
	where $\tilde{a}_1 = \min_i\{l_i>0\}, \tilde{a}_2 =(T+1) \max\{ \max_i \,l_i , \max_i \, b_i\}, \tilde{a}_3 = \max_i\{b_i^m\}, \rho = 1-\tilde{a}_1/\tilde{a}_2$. 
\end{enumerate}
\end{theorem}

\begin{example}
A combination of  $u$ together with $l,b,\mc X_f, \mc Z_f$ satisfying \eqref{eq:terminal-lyapunov} is as follows. Pick $u=\lambda$, let $l,b^r$ be arbitrary, $b^m_i\geq[(\IR)^{-1}l]_i/v_i, i\in[I], \xterm=x^{\text{up}}, \xterr=0$. For every $x\in\mc X_f, z^m\in\mc Z_f$, we have $x^r=0, f_i(x^m) = v_i x_i^m$, and $\xi(z^m_i)=0, i\in[I]$. Therefore, $b^\top \begin{bmatrix}
	F(x^m,z^m, u) - x^m \\ x^r-\lambda+\lambda-x^r
\end{bmatrix} = b^{m\top} \left(\lambda - (\IR) f(x^m) \right) \leq -l^\top x + b^{m\top}\lambda$, where the inequality follows from $b^m_i \geq[(\IR)^{-\top}l]_i/v_i$, $i\in[I]$. This inequality establishes the first condition in \eqref{eq:terminal-lyapunov}. The second condition follows from the proof of \Cref{prop:feasible-control-non-empty} in Appendix~\ref{proof:prop-feasibility}, where we show positive invariance of $\mc X_f$ under $u= \lambda$, and the positive invariance of $\mc Z_f$ follows similarly.
\end{example}










==> Traffic-adaptive-model-free-zl.tex <==
\section{Towards model-free settings}
\subsubsection{Stability Guarantees}

\begin{theorem}
	Let the inflow $\lambda$ satisfies $(\IR)^{-1}\lambda<\Cm$.
	Let $l(x) = 0$ for all $x\in\mc X_f$, and $l(x)=l$ for all $x\notin\mc X_f$ where $l$ is nonnegative and nonzero. 
	If the initial condition satisfies $x(0)\in\mc X\setminus\mc X_f$, then under the Set-PC control, there exists a finite time $K$ such that $x(K)\in\mc X_f$.
	Moreover, If the terminal set satisfies $\mc X_f\subseteq [0,\xunc]$, then the control $u(t) = \min \{ \max\{\bar{\lambda}(t), (\mathbf{I}-\bar{\mathbf{R}}(t))\ubar{C}^{\max}(t)\}, x^r(t) +\bar{\lambda}(t) \}$ locally stabilizes the system \eqref{eq:cell_compact_dynamic} in the sense that $||x(t)||<\infty$ for all $t\geq0$ and $x(0)\in\mc X_f$.
\end{theorem}
\begin{proof}	
	We proceed by showing that $\mathbbm{P}(\hat{x}(t), \hat{\theta}(t))$ is feasible $\implies$ $\mathbbm{P}(\bar{x}(t+1), \ubar{x}(t+1), \hat{\theta}(t))$ is feasible $\implies$ $\mathbbm{P}(\hat{x}(t + 1), \hat{\theta}(t+1))$ is feasible. It suffices to show that the terminal constraints $\mc X_f, \mc Z_f$ are satisfied since other constraints are satisfied by dynamics. Let $\{\hat{u}(0:T-1| t)\}$ denote a feasible solution to $\mathbbm{P}(\hat{x}(t), \hat{\theta}(t))$ and let $\tilde{u}(T) = 0$. We first show that the sequence $\{\hat{u}(1:T-1| t),\tilde{u}(T)\}$ is also a feasible solution to $\mathbbm{P}(\bar{x}(t+1), \ubar{x}(t+1), \hat{\theta}(t))$. From \eqref{eq:estimation}, $\bar{x}(t+1) = F(\xup(t), \xlb(t), u(t); \hat{\theta}(t))$. Therefore, $\Phi_x(\hat{x}(t), \hat{u}(0:k - 1| t); \hat{\theta}(t)) = \{\bar{x}(t+1), \Phi_x(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}(1:k| t); \hat{\theta}(t))\}$ for all $k=1,\ldots,T$. Since $\Phi_x(\hat{x}(t), \hat{u}(0:T-1| t); \hat{\theta}(t))\in\mc X_f$ and $\mc X_f$ is positively under the control $\tilde{u}(T)$, we have $\Phi_x(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}(1:T-1| t), \tilde{u}(T); \hat{\theta}(t))\in\mc X_f$. 
	
	Then, we show that $\{\hat{u}(1:T-1| t),\tilde{u}(T)\}$ is also a feasible solution to $\mathbbm{P}(\hat{x}(t + 1), \hat{\theta}(t+1))$. Since $\bar{\theta}(t+1) \leq \bar{\theta}(t), \ubar{\theta}(t+1)\geq\ubar{\theta}(t)$ and $\xup(t+1)\leq\bar{x}(t+1), \xlb(t+1) \geq \bar{x}(t+1)$, we have $\Phi_x(\hat{x}(t+1), \hat{u}(1:k-1| t); \hat{\theta}(t)) \leq \Phi_x(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}(1:k-1| t); \hat{\theta}(t))\in\mc X,\forall\, k\in[1:T]$ and $\Phi_x(\hat{x}(t+1), \hat{u}(1:k-1| t); \hat{\theta}(t))\in\mc X, \forall\, k\in[1:T]$ since $\mc X$ is box-constrained. Also, $\Phi_x(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}(1:T-1| t),\tilde{u}(T); \hat{\theta}(t))\in\mc X_f$ implies that $\Phi_x(\hat{x}(t), \hat{u}(0:T-1| t),\tilde{u}(T); \hat{\theta}(t))\in\mc X_f$ since $\mc X_f$ is box-constrained. The constraint satisfaction of $\mc Z_f$ follows similarly.
	
	For any feasible solution $\hat{u}(0:T-1| t)$, let $V(\hat{x}(t), \hat{u}(0:T-1| t), \hat{\theta}(t))$ denote the objective value of \eqref{eq:mpc-opt-adaptive}.
	 Let $V^*(\hat{x}(t), \hat{\theta}(t))$ denote the optimal value function of \eqref{eq:mpc-opt-adaptive}. Now we show that the value function $V^*(\hat{x}(t),\hat{\theta}(t))$ satisfies $V^*(\hat{x}(t + 1),\hat{\theta}(t+1)) - V^*(\hat{x}(t),\hat{\theta}(t)) \leq -l(\hat{x}(t))^T\hat{x}(t)$ so that the optimal objective value of \eqref{eq:mpc-opt-adaptive} decreases by at least $l(\hat{x}(t))^T\hat{x}(t)$ at each time step $t$. Let $\hat{u}^*(0:T-1| t)$ be an optimal solution to $\mathbbm{P}(\hat{x}(t),\hat{\theta}(t))$ and $\tilde{u}(T) = 0$. The sequence $\{\hat{u}^*(1:T-1| t),\tilde{u}(T)\}$ is also a feasible solution to $\mathbbm{P}(\hat{x}(t+1),\hat{\theta}(t+1)$ by the proof of recursive feasibility. Also, the objective function is monotone in $x$ and  $\Phi_x(\hat{x}(t+1), \hat{u}^*(1:k-1| t),\tilde{u}(T); \hat{\theta}(t)) \leq \Phi_x(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}^*(1:k-1| t),\tilde{u}(T); \hat{\theta}(t)),\forall\, k\in[1:T]$. Therefore, we have:
	\begin{equation}\label{eq:value-function-t-adaptive}
		\begin{split}
			&\quad\ V^*(\hat{x}(t+1), \hat{\theta}(t+1))\\&\leq V(\hat{x}(t+1), \hat{u}^*(1:T-1| t),\tilde{u}(T),\hat{\theta}(t+1)) \\ 
			& \leq V(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}^*(1:T-1| t),\tilde{u}(T),\hat{\theta}(t)) \\
		\end{split}
	\end{equation}
	This implies
	\begin{equation}\label{eq:value-function-inequality}
		\begin{aligned}
			&V^*(\hat{x}(t+1),\hat{\theta}(t+1)) - V^*(\hat{x}(t),\hat{\theta}(t)) \\
			\leq\ & V(\bar{x}(t+1),\ubar{x}(t+1), \hat{u}^*(1:T-1| t),\tilde{u}(T),\hat{\theta}(t)) \\ &\hspace{1in} -V(\hat{x}(t), \hat{u}^*(0:T-1| t),\hat{\theta}(t)) \\
			= \ & l(\Phi_x(\hat{x}(t),\hat{u}^*(0:T-1| t)))^T \Phi_x(\hat{x}(t),\hat{u}^*(0:T-1| t))	\\& \hspace{1.5in}- l(\xup(t))^\top\xup(t)\\
			= \ & -l(\xup(t))^\top\xup(t)
		\end{aligned}
	\end{equation} 
	where we use the inequality \eqref{eq:value-function-t-adaptive} and the fact that $\Phi_x(\hat{x}(t),\hat{u}^*(0:T-1| t))\in\mc X_f$ and $l(x)=0$ if $x\in\mc X_f$.
	
	Now we are ready to show that suppose $x(0)\notin\mc X_f$, there exists a finite time $K$ such that $x(K)\in\mc X_f$. For every $x\notin\mc X_f$, we have $l(x)^T x = l^T x\geq l^T \xterm>0$ and $l(x)^Tx = 0$ for all $x\in\mc X_f$. Let $\bar{t}$ denote a finite integer such that $\bar{t}l^T \xterm> V^*(\hat{x}(0), \hat{\theta}(0))$. Suppose the state has not entered $\mc X_f$ by time $t=\bar{t}$, we have $l(\xup(t))^T \xup(t)\geq l^T \xterm$ for $t\in[0:\bar{t}]$. From the telescoping sum of the inequality \eqref{eq:value-function-inequality} from $t=0$ to $\bar{t}-1$, we have $V^*(\hat{x}(\bar{t}),\hat{\theta}(t+1)) - V^*(\hat{x}(0),\hat{\theta}(0))\leq -\bar{t}l(\xup(t))^\top\xup(t) \leq -\bar{t}l^T \xterm$. This implies that $V^*(\hat{x}(\bar{t}),\hat{\theta}(t+1))\leq V^*(\hat{x}(0),\hat{\theta}(0)) -\bar{t}l^T \xterm <0 $, which contradicts the fact that $V^*(\hat{x}(\bar{t}),\hat{\theta}(t+1))$ is nonnegative. Therefore, $x(K)\in\mc X_f$ for some time $K\leq\bar{t}$.
	
	Then, we first  observe that $\bar{\lambda}(t)\equiv\lambda$ since $\lambda$ is assumed to be constant.
	From the proof of \cref{prop:feasible-control-non-empty}, we already showed that the uncongested region $[0,\xunc]$ is positively invariant under the control $u(t)=\lambda$. 
\end{proof}


==> Traffic-distributed-control-zl.tex <==
\section{Towards decentralized control settings}


 Both output-feedback model predictive and model-free controllers described in previous sections require available information all over the network to compute control inputs, which fit into the framework of centralized controllers. Next, we introduce a technique to design decentralized feedback control law inspired by \cite{Jafari.Savla:Automatica20}. 
 \begin{assumption}\label{ass:distributed}
 	We assume each cell can only access the information from itself and a few closest upstream and downstream cells. With the decentralized information, each cell computes its own control input accordingly. We denote by $\mc I_i$ the set of cell indices with available information for cell $i$.
 \end{assumption}
 

\begin{example}
	Consider the three-cell line segment in \Cref{ex:I-210-capacity}. One case that satisfies \Cref{ass:distributed} is as follows: $u_1(t)$ is computed based on information $y_1(t), y_2(t)$; $u_2(t)$ is computed based on information $y_1(t), y_2(t), y_3(t)$; $u_3(t)$ is computed based on information $y_2(t), y_3(t)$. That is, $\mc I_1=\{1,2\}, \mc I_2=\{1,2,3\}, \mc I_3=\{2,3\}$.
\end{example}

In MPC-set membership method \eqref{eq:estimation}, All steps except for MPC are inherently decentralized . Instead of the original optimiation problem \eqref{eq:mpc-opt}, we consider the following truncated optimization denoted by $\mathrm{P}_i(\hat{x}_{j\in\mc I_i}^m(t), \hat{z}_{j\in\mc I_i}^m(t), \hat{x}_{j\in\mc I_i}^r(t))$:

\begin{equation}\label{eq:mpc-opt-decentralized}
	\begin{aligned}
		&\minimize_{\substack{\hat{u}(0:T-1\mid t)}} \quad \sum_{k=0}^{T-1}l_{j\in\mc I_i}^\top x_{j\in\mc I_i}(k\mid t) + b_{j\in\mc I_i}^\top x_{j\in\mc I_i}(T\mid t) \\
		&\subjecto\\
		& x^m_i(k+1\mid t) = x^m_i(k\mid t) -f_i(x^m(k\mid t)) + u_i,\\ & \hspace{2in}\forall\, k \in[0,T-1]\\
		& x^m_j(k+1\mid t) = F_j(x^m(k\mid t),z^m(k\mid t),\hat{u}(k\mid t)),\\ & \hspace{1.5in}\forall\, k \in[0,T-1], \, j\in\mc I_i \backslash i\\
		& z^m_i(k+1\mid t) = z^m_i(k\mid t) -f_i(z^m(k\mid t)) + u_i,\\ & \hspace{2in}\forall\, k \in[0,T-1]\\
		&z_j^m(k+1\mid t) = F_j(z^m(k\mid t),x^m(k\mid t),\hat{u}(k\mid t)), \\ & \hspace{1.5in}\forall\, k \in[0,T-1],\, j\in\mc I_i \backslash i\\
		&x^r_j(k+1\mid t)  = x^r_j(k\mid t) - \hat{u}_j(k\mid t), \forall k \in[0,T-1], \, j\in\mc I_i\\
		&x(k\mid t) \in \mc X_{\mc I_i}, z^m(k\mid t) \in \mc X^m_{\mc I_i}, \hat{u}(k\mid t)\text{ satisfies \eqref{eq:u-constraint}}, \\ &\hspace{2.1in} \forall \, k\in[0:T-1] \\
		&x^m_j(0\mid t) = \hat{x}_j^m(t), z^m_j(0\mid t) = \hat{z}_j^m(t), x^r_j(0\mid t) = \hat{x}_j^r(t), \\ &\hspace{2.8in}
		\forall \, j\in\mc I_i \\
		%& x(T\mid t) \in \mc X_f, z^m(T\mid t) \in \mc Z_f \\
	\end{aligned}
\end{equation}
\begin{remark}
	In the truncated optimization \eqref{eq:mpc-opt-decentralized}, we omit the dependency on demand $\lambda$ and assume that there is no incoming flow to the network.
\end{remark}

As for the model-free control, we first reformulate the data matrices \eqref{eq:data} for each cell $i$ as follows:
\begin{equation}\label{eq:data-distributed}
	\begin{aligned}
		\U_{i}(t-1) &:= \\ & 
			\begin{bmatrix}
			u_{ j\in \mc I_i}(t-L-1) &  \ldots &  u_{j\in \mc I_i}(t-1) 
		\end{bmatrix}\in \real^{\lvert\mc I_i\rvert \times L}\\
		\Y_{i}(t) &:= \\ &\begin{bmatrix}
		y_{j\in\mc I_i}(t-L) &  \ldots   &y_{j\in\mc I_i}(t) \\
		\end{bmatrix}\in\real^{\lvert\mc I_i\rvert\times L} \\
		\Z_i(t-1) &:=\\ &
		\begin{bmatrix}
				y_{j\in\mc I_i}(t-L-1)  & \ldots& y_{j\in\mc I_i}(t-1)  \\
				r_1  & \ldots& r_L
		\end{bmatrix}\in\real^{(\lvert\mc I_i\rvert+1)\times L}
	\end{aligned}
\end{equation}
Then, the decentralized control law is defined as follows:
\begin{equation}\label{eq:data-driven-distributed-control}
	\begin{aligned}
		&u_i(t)=
		\min\Big\{\bar{u}_i,  \\ & \hspace{0.1in}\max\big\{0,\big[ \K(\U_i(t-1),\Y_i(t),\Z_i(t-1))\begin{bmatrix}	y_{j\in\mc I_i}(t) \\ r_L  \end{bmatrix}\big]_i\big\}\Big\} \\ & \hspace{1.6in} +\epsilon_i(t)\lVert y_{j\in\mc I_i}(t) \rVert_1, \, i\in [I]
	\end{aligned}
\end{equation} 
where the output-feedback gain is defined in \eqref{eq:data-driven-control} and \eqref{eq:sdp-data}. 

==> Traffic-model-free-zl.tex <==
\section{Towards model-free settings}

MPC-set membership method does not require complete state information but the exact knowledge of model parameters. Therefore, a natural next step is to pursue the design of a controller that directly takes measured outputs to compute control inputs accordingly without knowing any parameters and thus becomes a \emph{model-free} controller. 


To achieve this, we modify the output model \eqref{eq:output_measurements} by removing all zero elements in $y^m(t)$ and accordingly zero rows in $\mathbf{C}$. Let $I_c$ denote the number of remaining rows in $\C$, which equals the number of cells with available outputs. 
%Let $\tilde{\mathbf{C}}\in\real^{I_c\times 2I}$ denote the modifed $\C$ accordingly.
Then, we extend the idea of approximate nonlinearity cancellation in \cite{de2023learning}, which focuses on state-feedback static controllers. Here, we design an online updated controller that only depends on output data.

Let $L$ be a time horizon within which data are available. For $t\in[0,L]$, we assume control $u(t)$ are given.
At every time $t\geq L+1$, we collect measurements and inputs of the system over the past $L+1$ time steps in appropriate matrices of data as follows:
\begin{equation}\label{eq:data}
	\begin{aligned}
		\U_{t-1} &:= \left[u(t-L-1)\quad  \ldots \quad  u(t-1)\right]\in \real^{I\times L} \\
		\Y_{t} &:= \left[y(t-L)\hspace{0.4in}  \ldots  \quad y(t)\right]\in\real^{I_c\times L} \\
		\Z_{t-1} &:=\!\left[
		\begin{aligned}
			&y(t-L-1)  && \ldots\ &&& y(t-1)  \\
			&r_1  && \ldots\ &&& r_L
		\end{aligned}
		\right]\in\real^{(I_c+1)\times L}
	\end{aligned}
\end{equation}
where $r_1\ldots r_L$ are predetermined fixed but different numbers.
\begin{remark}\label{remark:Q}
	\cite{de2023learning} constructs the matrix $\Z$ by combing state information $x(0)\ldots x(L-1)$ with nonlinearity $Q(x(0)) \ldots Q(x(L-1))$ where $Q(x)$ contains known nonlinear functions. It is known that the CTM can be reformulated as piecewise affine systems for which $Q(x)$ equals a constant that depends on if $x_i$ is congested or not for all $i\in[I]$. Since $\xcrit$ is assumed to be unknown, $Q(x)$ is also unknown. Instead, we put different constant numbers $r_1\ldots r_L$ into account that switches between uncongested and congested states may happen at every time step.
\end{remark}

With available data \eqref{eq:data},
we propose the following feedback control law:
\begin{equation}\label{eq:data-driven-control}
	\begin{aligned}
		u_i(t)=
		&\min\Big\{\bar{u}_i, \max\big\{0, \big[ \K(\U_{t-1},\Y_t,\Z_{t-1})\begin{bmatrix}	y(t) \\ r_L  \end{bmatrix}\big]_i\big\}\Big\} \\ & \hspace{1.6in}+ \epsilon_i(t)\lVert y(t) \rVert_1, \, i\in [I]
	\end{aligned}
\end{equation} 
where $\K(\U_{t-1},\Y_t,\Z_{t-1})\in\real^{I\times (I_c+1)}$ is the output-feedback gain and $\epsilon(t)$ is an auxiliary input signal that belongs to the ball
\begin{equation}
	\mc B_\delta := \{\epsilon\in\real^I:\lVert\epsilon\lVert_2 \leq\delta\}
\end{equation}
for every time $t$ and some sufficiently small $\delta>0$. Following \cite{de2023learning}, we define the feedback gain as 
\begin{equation}
	\K(\U_{t-1},\Y_t,\Z_{t-1})= \U_{t-1}[\W\PP^{-1} \quad \G]
\end{equation}
with $\PP\in\mathbb{S}^{I_c\times I_c},\W\in\real^{L\times I_c},\G\in\real^{L\times 1}$
computed by the following semi-definite program (SDP):
\begin{equation}\label{eq:sdp-data}
	\begin{aligned}
		\minimize_{\PP,\W,\G}\quad &\lVert \Y_t \G \rVert_2 \\
		\subjecto \quad& \Z_{t-1}\W = \begin{bmatrix}	\PP \\ 0_{1\times I_c}	\end{bmatrix} \\
		& \begin{bmatrix}
			\PP & (\Y_t\W)^\top \\
			\Y_t\W & \PP
		\end{bmatrix}\succ 0 \\
		& \Z_{t-1}\G = \begin{bmatrix}
			0_{I_c\times 1} \\ 1
		\end{bmatrix}
	\end{aligned}
\end{equation}
where $\succ$ denotes positive definiteness.
When $\C=\mathbf{I}$, the closed-loop system \eqref{eq:cell_dynamics}, \eqref{eq:output_measurements} in feedback with \eqref{eq:data-driven-control} behaves similarly to the form
\begin{equation}\label{eq:data-closed-loop}
	x(t+1) = \Y_t\W\PP^{-1}x(t) + \Y_t\G Q(x(t))
\end{equation}
where $Q(x(t))$ is a scalar nonlinear function (cf. \Cref{remark:Q}).
The objective function $\lVert \Y_t \G \rVert_2$ corresponds to coefficients of the nonlinearity in \eqref{eq:data-closed-loop}, and thus \eqref{eq:sdp-data} minimizes the nonlinearity. The constraints in \eqref{eq:sdp-data} are designed to reach the form \eqref{eq:data-closed-loop} and ensure that the remaining linear dynamics $x(t+1) = \Y_t\W\PP^{-1}x(t)$ are stable. 
\begin{remark}
	The control law \eqref{eq:data-driven-control} does not satisfy \eqref{eq:u-constraint}. As a result, we directly deal with data from \eqref{eq:cell_dynamics} instead of the simplified dynamics \eqref{eq:cell_compact_dynamic}.
\end{remark}
\begin{remark}\label{remark:data-feasibility}
	A necessary condition for the SDP \eqref{eq:sdp-data} to be feasible is that $Z_{t-1}$ has full row rank. Such a requirement can be viewed as a condition on the richness of data as mentioned in \cite{de2023learning}. Therefore, control inputs $u(t), t\in[0,L]$ need to be selected carefully to excite the system and obtain rich enough data from the system.
	The auxiliary input signal $\epsilon(t)$ is also proposed for $u(t)$ to excite the system as suggested by \cite{rotulo2022online}. The bound $\delta$ can take any values below an upper bound $\delta\leq\bar{\delta}$ of which the exact value depends on dynamics but is not needed for computation (cf. Remark~2 in \cite{rotulo2022online}). 
\end{remark}

In \Cref{sec:simulations}, simulations suggest that the proposed model-free controller stabilizes traffic in the sense that the total number of vehicles remains bounded. A rigorous proof of the input-to-state stability similar to \Cref{theo:ISpS} is in progress.




==> performance-guarantees-mpc-mhe-ks.tex <==
\subsection{Performance Guarantee of the MPC-MHE Controller}
We now find sufficient conditions under which the MPC-MHE controller is stabilizing. Following \cite{copp2017simultaneous}, this relates to the existence of saddle-point for the min-max problem in \eqref{eq:min-max}. 


\begin{theorem} \label{theo:existence_saddle}
Let Assumption \ref{ass:C-matrix} and \ref{ass:terminal-constraints} be true. \zl{Suppose that all elements in $l^m$ and $b^m$ are equal}. For given input sequence $u(t-L:t-1)$, output sequence $y(t-L:t)$, and inflow rates $\lambda$ at the ramps, there exists a mainline initial condition $x^{\circ,m,*}\in\mathcal{X}^m$ and future \zl{input} sequence $\hat{u}^*(t:t+T-1)$ such that
	\begin{equation}\label{eq:saddle_point}
		\begin{aligned}
			&J_t(x^{\circ,m,*},\hat{u}^*(t:t+T-1)) \\ & \hspace{0.5in}= \min_{\substack{\hat{u}(t:t+T-1)\in\mc{U}}} \, J_t(x^{\circ,m,*},\hat{u}(t:t+T-1))\\
			& \hspace{1in}= \max_{x^{\circ,m}\in\mathcal{X}^m} J_t(x^{\circ,m},\hat{u}^*(t:t+T-1)) 
		\end{aligned}
	\end{equation}
\end{theorem}
\begin{proof}
	The proof is given in Appendix~\ref{proof:theo-existence-saddle-points}.
\end{proof}
\ksmargin{polish the language of the Remark}
\zl{
\begin{remark}
%\begin{enumerate}
%\item 
\cite{copp2016conditions} proposes a sufficient condition for the existence of saddle-points and requires observability and proper choices of cost functions in the case of linear time-invariant systems. Their analysis requires the objective function to be convex with respect to control inputs and concave with respect to initial conditions. However, this does not generally hold true for nonlinear systems. \cite{schmitt2020convexity} explored the existence of saddle-points for robust control of traffic systems under uncertain parameters. They consider known initial conditions with certainty and claim that it is hard and not pursued to consider uncertain initial states. \cite[Remark 2]{schmitt2020convexity}. Our work utilizes the properties of the set of feasible initial conditions and control inputs and extends the idea in \cite{schmitt2020convexity} to the case of unknown initial states.
%\end{enumerate}
\end{remark}
}

\zl{Unlike objective functions in standard MPC defined as the difference between the current state and the desired equilibrium state, the objective defined in \eqref{eq:finite-horizon-cost} represents the total number of vehicles and characterizes the system performance or profits, which is in line with economic MPC. Therefore, as for cost coefficients and terminal constraints, we make the following assumption inspired by the assumption of economic MPC \cite{rawlings2012fundamentals} which is different from the assumption made in the original MPC-MHE \cite{copp2017simultaneous}. Let $\phi(x, u)$ denote the state values after one-step evolution starting from $x$ given $u$ under \eqref{eq:cell_compact_dynamic}, we assume:
	\begin{assumption} \label{assu:obj_lyapunov}
		%Consider the traffic dynamics \eqref{eq:cell_compact_dynamic}, 
		For every $\lambda \geq 0$ satisfying \eqref{eq:max-flow}, there exists a control $u$ satisfying \eqref{eq:u-constraint} such that for every $x\in\mathcal{X}_f$, the following holds under \eqref{eq:cell_compact_dynamic}:
		\begin{equation}\label{eq:obj_lyapunov}
			b^\top \phi(x, u) - b^\top x \leq -l^\top x + l^\top x^{unc}(\lambda)
		\end{equation}
	\end{assumption}
	\begin{example}
		Let $v$ denote the vector of parameters $v_i, i\in[I]$ and $\odot$ denote the component-wise multiplication. An example of $\mathcal{X}_f$, $l$ and $b$ that satisfy the assumption is that $\mc X_f$ is defined by \eqref{eq:terminal_constraints}, 
			$l^m\geq l^r$, $b^m\odot v=(\mathbf{I}-\mathbf{R})^{-\top}l^m$ and $b^r\odot v=(\mathbf{I}-\mathbf{R})^{-\top}l^r$.  The terminal constraints require every mainstream cell is uncongested and the length of all on-ramp queues is zero. The assumption can be verified as follows. For every $x\in\mathcal{X}_f$, we have $x^r=0$ and $f(x^m) = v\odot x^m$. Therefore, let $u=0$ from \eqref{eq:cell_compact_dynamic} we have 
			\begin{multline}
				b^\top \phi(x, u) - b^\top x = b^{r\top}\lambda - b^{m\top} (\mathbf{I}-\mathbf{R})f(x^m)\\
				= b^{r\top}(\mathbf{I}-\mathbf{R})f^{eq}(\lambda) - b^{m\top} (\mathbf{I}-\mathbf{R})f(x^m)  \\
				= b^{r\top}(\mathbf{I}-\mathbf{R})f(x^{unc}(\lambda)) - b^{m\top} (\mathbf{I}-\mathbf{R})f(x^m)\\
				\leq l^{m\top} x^{unc}(\lambda) - l^{m\top} x^m = -l^\top x + l^\top x^{unc}(\lambda)
			\end{multline}
			The last inequality holds if  $b^m\odot v=(\mathbf{I}-\mathbf{R})^{-\top}l^m$, $b^r\odot v=(\mathbf{I}-\mathbf{R})^{-\top}l^r$ and $l^m\geq l^r$ because all elements in $(\mathbf{I}-\mathbf{R})^{-\top}$ are nonnegative \cite{schmitt2020convexity}.
		\end{example}
	}

==> proof-Maximal-element-LP-ks.tex <==
\subsection{Proof of Proposition~\ref{prop:maximal-element-LP}}
\label{proof:maximal-element-LP}
%First, we show that the matrix $(\RJ)^{-1}$ exists and is nonnegative. It is observed that such a matrix lies in the class of $\mathbf{Z}$-matrix \cite{fiedler1962matrices} defined as follows:
%\begin{definition}\label{def:z-matrix}
%	A square matrix is said to be a $\mathbf{Z}$-matrix if its off-diagonal elements are all non-positive.
%\end{definition}
%
%The class of $\mathbf{Z}$-matrix has the following properties.
%
%\begin{lemma}\label{lemm:z-matrix-inverse}
%	Let $\mathbf{A}$ be an $\mathbf{Z}$-matrix. Then the following conditions are equivalent:
%	\begin{enumerate}
%		\item There exists a vector $x\geq 0$ such that $\mathbf{A}x> 0$.
%		\item The inverse $\mathbf{A}^{-1}$ exists and all elements in $\mathbf{A}^{-1}$ are nonnegative.
%	\end{enumerate}
%\end{lemma}
\eqref{eq:cell-augmented-dynamics} implies that $\tilde{\mathbf{R}}$ is a $Z$-matrix. 
%\begin{equation*}
$\tilde{\mathbf{R}} \begin{bmatrix} x^m \, \, x^a \end{bmatrix}^{\top}
=\begin{bmatrix} x^m_1 - x^m_2 \, \, \beta_1 x_2^m - x_3^m \, \, \beta_2 x_3^m - x_4^m \, \, \ldots \, \, \beta_{I-1} x^m_I - x^a \, \, \beta_I x^a\end{bmatrix}^{\top}$, 
%\end{equation*}
from which \kscomment{one can easily see construct $[x^m \, \, x^a]^{\top} \geq 0$ such that $\tilde{\mathbf{R}} \begin{bmatrix} x^m \, \, x^a \end{bmatrix}^{\top} > 0$.}  Therefore, Lemma~\ref{lemm:z-matrix-inverse} implies that $\tilde{\mathbf{R}}^{-1}$ exists and all its elements are nonnegative. \eqref{eq:cell-augmented-dynamics} can be equivalently written as:
\begin{equation*}\label{eq:constraint-augmented-transform}
	\tilde{\mathbf{R}}^{-1}\begin{bmatrix}x^m(s+1)\\x^{a}(s+1)\end{bmatrix} =\tilde{\mathbf{R}}^{-1}\begin{bmatrix} x^m(s) \\0 \end{bmatrix}   + \tilde{f}(s) + \tilde{\mathbf{R}}^{-1} \begin{bmatrix} u_1(s)\\ \vdots \\ u_I(s) \\ 0\end{bmatrix}
\end{equation*} \ksmargin{why?}
An optimal solution to \eqref{eq:lp-maximal} must satisfy \eqref{eq:flow-augmented}. If this is not the case, e.g., $\tilde{f}_{i+1}(s)<f_i(x^m(s))$ for some $i \in I$, $s \in [t-L:t-1]$, then replacing $\tilde{f}_{i+1}(s)$ with $f_i(x^m(s))$ is a \kscomment{strictly better solution.} The result now follows from the fact that $\tilde{\mathbf{R}}^{-1}$ is nonnegative and therefore 
%\begin{equation*}
	\kscomment{$\tilde{\mathbf{R}}^{-1}\begin{bmatrix}
		\hat{x}^{\circ,m} \\ f_I(\hat{x}^{\circ,m})
	\end{bmatrix}\succ\tilde{\mathbf{R}}^{-1}\begin{bmatrix}
		x^{\circ,m} \\ f_I(x^{\circ,m})
	\end{bmatrix}$ 
%\end{equation*} 
for all $x^{\circ,m}\in\mc X^m$.} \ksmargin{need more details here} 

==> proof-U-equiv-ks.tex <==
\subsection{Proof of Proposition~\ref{prop:U-equiv}}
\label{proof:U-equiv}
\zl{
The proposition follows once we show that $(\hat{x}^{\circ,m},\hat{z}^{\circ,m})$ is the maximal/minimal element in $\mc X_{t_1:t_2}^{\circ,m}$, i.e., \zl{$\hat{x}^{\circ,m}\geq x^{\circ,m}, \hat{z}^{\circ,m}\leq z^{\circ,m}$} for all $(x^{\circ,m}, z^{\circ,m})\in\mc X_{t_1:t_2}^{\circ,m}$. This is because $\tilde{\mc U}_{t_1:t_2}(T;\hat{x}^{\circ,m},\hat{z}^{\circ,m})\subseteq\mc U_{t_1:t_2}(T)$ then follows from the monotonicity property in Lemma~\ref{lemm:embedding-system} and $\tilde{\mc U}_{t_1:t_2}(T;\hat{x}^{\circ,m},\hat{z}^{\circ,m})=\tilde{\mc U}_{t_1:t_2}(T;\hat{z}^{\circ,m},\hat{x}^{\circ,m})$. The latter is because $x^{\circ,m}$ and $z^{\circ,m}$ are interchangeable in $\mc X_{t_1:t_2}^{\circ,m}$ and constraints on mainline states $x^m$ and $z^m$ are the same in $\tilde{\mc U}_{t_1:t_2}(T;x^{\circ,m},z^{\circ,m})$. 
 
% The following result for the set of feasible initial conditions defined in \eqref{eq:X-def} uses Lemma~\ref{lemm:maximal_X}. 
%	
%	\begin{lemma}\label{lemm:maximal_element}
%		Let Assumption \ref{ass:C-matrix} be true. 
%		For every state trajectory on the ramps $x^r(t-L:t)$, 
%		input sequence $u(t-L:t-1)$,  
%		output sequence $y(t-L:t)$, there exists a unique $\hat{x}^{\circ, m}$ such that $\hat{x}^{\circ,m}\geq x^m$ for all $x^{\circ,m}\in \mc X^m(x^r(t-L:t), u(t-L:t-1),y(t-L:t))$.
%	\end{lemma} 
	
%For brevity, we simply write $\mc X^m$ for the set under consideration. 
$\mc X^{\circ,m}_{t_1:t_2}$ is compact by definition in \eqref{eq:X-def}.  Therefore, following Lemma~\ref{lemm:maximal_X}, we just need to show that $\mc X^{\circ,m}_{t_1:t_2}$ is closed with respect to componentwise maximization for $x^{\circ,m}$ and minimization for $z^{\circ,m}$. Consider $(x^{\circ,m,1},z^{\circ,m,1}) \in \mc X^{\circ,m}_{t_1:t_2},(x^{\circ,m,2},z^{\circ,m,2}) \in \mc X^{\circ,m}_{t_1:t_2}$, such that $(x^{\circ,m,1},z^{\circ,m,1})\neq (x^{\circ,m,2},z^{\circ,m,2})$. Let $(x^{\circ,m},z^{\circ,m} ):=\big(\max\{x^{\circ,m,1},$
$ x^{\circ,m,2}\},\min\{z^{\circ,m,1}, z^{\circ,m,2}\}\big)$ be the elementwise maximum/minimum. We first show by induction on $t$ that the trajectories \zl{$\Phi^{t,x,m}_{t_1}\left( x^{\circ,m}, z^{\circ,m},u(t_1:t-1)\right) \equiv x^m(t)$} satisfy \eqref{eq:output-embedding-traffic} and $x^m(t)\leq \bar{x}$ for $t=t_1,\ldots,t_2$. The constraints corresponding to $ \Phi^{t,z,m}_{t_1}\left( x^{\circ,m}, z^{\circ,m},u(t_1:t-1)\right) \equiv z^m(t)$ can be handled similarly. Let the notations $x^{m,1}(t)$, $x^{m,2}(t)$,  $z^{m,1}(t)$, and $z^{m,2}(t)$ be defined similarly. 
		
		For a cell $i$ with $c_{i,i}\neq 0$, we have $y_i(t_1) = c_{i,i}x_i^{m,1}(t_1) = c_{i,i}x_i^{m,2}(t_1)$, giving $x_i^{m,1}(t_1)=x_i^{m,2}(t_1)=x^{m}(t_1)$, where the last equality follows from the definition of $x^{m}$. Similarly, $z_i^{m,1}(t_1)=z_i^{m,2}(t_1)=z^{m}(t_1)$. Therefore, \eqref{eq:embedding-traffic} gives:
\begin{equation*}
			\begin{aligned}
				x^m_i(t_1+1) = \, x^m_i(t_1) &+ \min\left\{\beta_{i-1}\ms d_{i-1}(x_{i-1}^{m}(t_1), z_{i-1}^{m}(t_1)), \beta_{i-1}s_i(x_i^m)(t_1)\right\} \\ & - \min\left\{\ms d_{i}(x_i^m(t_1),x_i^m(t_1)), s_{i+1}(x_{i+1}^m(t_1)) \right\} + u_i(t_1)
			\end{aligned}
		\end{equation*}		
		
		%Then we show that $y_i(t-L+1) =  c_{ii}\hat{x}_i(t-L +  1)$. 
		Since $c_{i,i}x_i^{m,1}(t_1 + 1) = c_{i,i}x_i^{m,2}(t_1 + 1)$, we have $x_i^{m,1}(t_1+1) = x_i^{m,2}(t_1+1)$ and similarly $z_i^{m,1}(t_1+1) = z_i^{m,2}(t_1+1)$. Therefore,  following \eqref{eq:embedding-traffic}:
		\begin{equation}
			\label{eq:lemma2-interim-1}
			\begin{aligned}
				& \min\left\{\beta_{i-1}\ms d_{i-1}\left(x^{m,1}_{i-1}(t_1), z_{i-1}^{m,1}(t_1)\right), \beta_{i-1}s_i\left(x_i^{m,1}(t_1)\right)\right\} - \min\left\{\ms d_i\left(x_i^{m,1}(t_1),x_i^{m,1}(t_1)\right), s_{i+1}\left(x_{i+1}^{m,1}(t_1)\right)\right\} \\
				&=\min\left\{\beta_{i-1}\ms d_{i-1}\left(x^{m,2}_{i-1}(t_1), z_{i-1}^{m,2}(t_1)\right), \beta_{i-1}s_i\left(x_i^{m,2}(t_1)\right)\right\} - \min\left\{\ms d_i\left(x_i^{m,2}(t_1),x_i^{m,2}(t_1)\right), s_{i+1}\left(x_{i+1}^{m,2}(t_1)\right)\right\}
			\end{aligned}
		\end{equation} 
		Following Assumption~\ref{ass:C-matrix}, let $c_{i-1,i-1} \neq 0$, i.e.,  $x^{m,1}_{i-1}(t_1) = x^{m,2}_{i-1}(t_1),z^{m,1}_{i-1}(t_1) = z^{m,2}_{i-1}(t_1)$; $d_{i-1,i-1}\neq 0$ can be handled similarly. Using $x^{m,1}_i(t_1) = x^{m,2}_i(t_1)$ in \eqref{eq:lemma2-interim-1}, we have that 
			\begin{equation*}
				\begin{aligned}
					 \min\left\{\ms d_i\left(x_i^{m,1}(t_1),x_i^{m,1}(t_1)\right), s_{i+1}\left(x_{i+1}^{m,1}(t_1)\right)\right\}  & =\min\left\{\ms d_i\left(x_i^{m,2}(t_1),x_i^{m,2}(t_1)\right), s_{i+1}\left(x_{i+1}^{m,2}(t_1)\right)\right\}
					\\ & = \min\left\{\ms d_i\left(x_i^{m}(t_1),x_i^{m}(t_1)\right), s_{i+1}\left(x_{i+1}^{m}(t_1)\right)\right\}
				\end{aligned}
			\end{equation*}
		where the last equality again follows from the definition of $x^m$, since $x_i^{m,1}(t_1)=x_i^{m,2}(t_1)=x^{m}(t_1)$ and $s_{i+1}\left(x_{i+1}^{m}(t_1)\right)$ is the minimum of $s_{i+1}\left(x_{i+1}^{m,1}(t_1)\right)$ and $s_{i+1}\left(x_{i+1}^{m,2}(t_1)\right)$. Therefore, \eqref{eq:lemma2-interim-1} is equal to 
		\begin{equation*}
				\min\left\{\beta_{i-1}\ms d_{i-1}\left(x_{i-1}^m(t_1), -z_{i-1}^m(t_1)\right), \beta_{i-1}s_i\left(x_i^{m}(t_1)\right)\right\} - \min\left\{\ms d_i\left(x_i^m(t_1), x_i^m(t_1)\right), s_{i+1}(x_{i+1}^m(t_1))\right\}
		\end{equation*}
	 Following \eqref{eq:cell_dynamics}, this implies that $x^{m,1}_i(t_1+1)=x^{m,2}_i(t_1+1)=\Phi_{t_1}^{t_1+1,x,m}(x_i^m(t_1),z_i^m(t_1),u(t_1))=:x_i^m(t_1+1)$. Similarly, $z_i^{m,1}(t_1 + 1) = z_i^{m,2}(t_1+1) =z_i^{m}(t_1+1)$.
		
%		Then we show that $x^m(s)\leq \bar{x}$ for $s = t-L, \ldots, t$. For any cell $i$ with $c_{i,i} > 0$, we have that $x^m_i(s)\leq \bar{x}_i$. 
		For a cell $i$ with $c_{i,i}=0$, following Assumption~\ref{ass:C-matrix}, we first consider $c_{i+1,i+1}\neq 0$ and $c_{i-1,i-1}\neq 0$. Following similar analysis as above, these respectively imply that $x^{m,1}_{i+1}(t_1)=x^{m,2}_{i+1}(t_1)=x^{m}_{i+1}(t_1);\, z^{m,1}_{i+1}(t_1)=z^{m,2}_{i+1}(t_1)=z^{m}_{i+1}(t_1)$ and $x^{m,1}_{i-1}(t_1)=x^{m,2}_{i-1}(t_1)=x^{m}_{i-1}(t_1);\, z^{m,1}_{i-1}(t_1)=z^{m,2}_{i-1}(t_1)=z^{m}_{i-1}(t_1)$. Therefore, 
		\begin{multline*}
			x^m_i(t_1+1) = x^m_i(t_1) + \beta_{i-1}f^{\text{in}}_{i}(x^{m}(t_1),z^m(t_1)) - f_{i}(x^{m}(t_1)) \\=\max\left\{x^{m,1}_i(t_1),x^{m,2}_i(t_1)\right\} + \beta_{i-1}\min\left\{\ms d_{i-1}(x_{i-1}^m,z_{i-1}^m), s_i\left(\max\left\{x^{m,1}_i(t_1),x^{m,2}_i(t_1)\right\}\right)\right\} - \\ \min\left\{\ms d_i\left(\max\left\{x^{m,1}_i(t_1),x^{m,2}_i(t_1)\right\},\max\left\{x^{m,1}_i(t_1),x^{m,2}_i(t_1)\right\}\right),s_{i+1}\left(x^m_{i+1}(t_1)\right)\right\} \\=\max\left\{x^{m,1}_i(t_1+1),x^{m,2}_i(t_1+1)\right\}\leq \bar{x}_i.
		\end{multline*}
	If $d_{i-1,i-1}\neq 0$ and $d_{i,i}\neq 0$, then $f^\text{in}_i\left(x^{m,1}(t_1), z^{m,1}(t_1)\right) = f^\text{in}_i\left(x^{m,2}(t_1), z^{m,2}(t_1)\right)=f^\text{in}_i\left(x^{m}(t_1), z^{m}(t_1)\right),$ $ f_i\left(x^{m,1}(t_1)\right) = f_i\left(x^{m,2}(t_1)\right)=f_i\left(x^{m}(t_1)\right)$, and hence $x^m_i(t_1+1) = \max\left\{x^{m,1}_i(t_1),x^{m,2}_i(t_2)\right\} + \beta_{i-1}f^{\text{in}}_{i}(x^{m}(t_1),z^m(t_1)) - f_{i}(x^{m}(t_1)) =\max\left\{x^{m,1}_i(t_1+1),x^{m,2}_i(t_1+1)\right\} \leq \bar{x}_i$. Similarly, $z_i^m(t_1+1) = \min\left\{z_i^{m,1}(t_1), z_i^{m,2}(t_2)\right\}\leq \bar{x}_i$.
	
	For a cell $i\in[I-1]$ with $d_{i,i}\neq0$, following \Cref{ass:C-matrix}, first let $c_{i,i}\neq 0, c_{i+1,i+1} = 0$. Following similarly analysis as above, this implies that
		$x^{m,1}_i(t_1+1)=x^{m,2}_i(t_1+1) = x^m_i(t_1+1), x^{m}_{i+1} = \max\left\{x^{m,1}_{i+1}(t_1+1),x^{m,2}_{i+1}(t_1+1)\right\},$ $ z_i^{m,1}(t_1 + 1) = z_i^{m,2}(t_1+1) =z_i^{m}(t_1+1),$ and therefore $f^{\text{in}}_{i+1}\left(x^{m}(t_1+1),z^{m}(t_1+1)\right) = f_i(x^{m}(t_1+1) = \min\big\{f_i\left(x^{m,1}(t_1+1)\right),$  $f_i\left(x^{m,2}(t_1+1)\right)\big\}$. From $y^f_i(t_1+1) = d_{i,i}f_i\left(x^{m,1}(t_1+1)\right) = d_{i,i}f_i\left(x^{m,2}(t_1+1)\right)$, we have $f_i\left(x^{m,1}(t_1+1)\right) = f_i\left(x^{m,2}(t_1+1)\right)  = f_i(x^{m}(t_1+1)  = f^{\text{in}}_{i+1}\left(x^{m}(t_1+1),z^{m}(t_1+1)\right)$. Then, let $c_{i,i} = 0, c_{i+1,i+1}\neq0$, again this implies $x^{m,1}_{i+1}(t_1+1)=x^{m,2}_{i+1}(t_1+1) = x^m_i(t_1+1),x^{m}_{i} = \max\left\{x^{m,1}_{i}(t_1+1),x^{m,2}_{i}(t_1+1)\right\},$ $ z^{m}_{i} = \min\left\{z^{m,1}_{i}(t_1+1),z^{m,2}_{i}(t_1+1)\right\}$, and \eqref{eq:embedding-traffic} gives
		\begin{equation}\label{eq:proof-flow-equality}
			\begin{aligned}
				\dfrac{y^f_i(t_1+1)}{d_{i,i}} &= \min\left\{\ms d_i\left(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1)\right),s_{i+1}\left(x_{i+1}^{m}(t_1+1)\right)\right\} \\ &= 	\min\left\{\ms d_i\left(x_i^{m,2}(t_1+1),z_i^{m,2}(t_1+1)\right),s_{i+1}\left(x_{i+1}^{m}(t_1+1)\right)\right\} \\
				&=	\min\left\{\ms d_i\left(x_i^{m,1}(t_1+1),x_i^{m,1}(t_1+1)\right),s_{i+1}\left(x_{i+1}^{m}(t_1+1)\right)\right\} \\ &=	\min\left\{\ms d_i\left(x_i^{m,2}(t_1+1),x_i^{m,2}(t_1+1)\right),s_{i+1}\left(x_{i+1}^{m}(t_1+1)\right)\right\} = \dfrac{y^{f^\text{in}}_i(t_1+1)}{\tilde{d}_{i+1,i+1}}.
			\end{aligned}
		\end{equation}
	Suppose $\dfrac{y^f_i(t_1+1)}{d_{i,i}} \neq \min\{\ms d_i(x_i^{m}(t_1+1),z_i^{m}(t_1+1)),s_{i+1}(x_i^{m}(t_1+1))\} $. Since $\ms d_i(x_i^{m}(t_1+1),z_i^{m}(t_1+1))\geq \ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1)), \ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1))\geq s_{i+1}(x_{i+1}^{m}(t_1+1))$ results in equality. Consider $\ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1))< s_{i+1}(x_{i+1}^{m}(t_1+1))$, then  $\dfrac{y^f_i(t_1+1)}{d_{i,i}}  = \ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1)) $, and we have the following two cases:
	\begin{enumerate}
		\item $\ms d_i(x_i^{m,1}(t_1+1),x_i^{m,1}(t_1+1))\leq s_{i+1}(x_{i+1}^{m}(t_1+1))$: \eqref{eq:proof-flow-equality} gives $\xi(x^{m,1}_i(t_1+1)) = \xi(z^{m,1}_i(t_1+1))$. If $\ms d_i(x_i^{m,2}(t_1+1),x_i^{m,2}(t_1+1))\leq s_{i+1}(x_{i+1}^{m}(t_1+1))$, then $\xi(x^{m,1}_i(t_1+1)) = \xi(z^{m,1}_i(t_1+1)) = \xi(x^{m,2}_i(t_1+1)) = \xi(z^{m,2}_i(t_1+1))$, and therefore $\ms d_i(x_i^{m}(t_1+1),z_i^{m}(t_1+1)) = \ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1)) $. If $\ms d_i(x_i^{m,2}(t_1+1),x_i^{m,2}(t_1+1))> s_{i+1}(x_{i+1}^{m}(t_1+1))$, then \eqref{eq:proof-flow-equality} is violated.
		\item $\ms d_i(x_i^{m,1}(t_1+1),x_i^{m,1}(t_1+1))> s_{i+1}(x_{i+1}^{m}(t_1+1))$: \eqref{eq:proof-flow-equality} gives $\dfrac{y^f_i(t_1+1)}{d_{i,i}} =s_{i+1}(x_{i+1}^{m}(t_1+1))$ which contradicts  $\ms d_i(x_i^{m,1}(t_1+1),z_i^{m,1}(t_1+1))< s_{i+1}(x_{i+1}^{m}(t_1+1))$.
	\end{enumerate}
Since $(x_i^{m,1}(t_1+1), z_i^{m,1}(t_1+1))$ and  $(x_i^{m,2}(t_1+1), z_i^{m,2}(t_1+1))$ are interchangeable in the analysis above, we have  $\dfrac{y^f_i(t_1+1)}{d_{i,i}} = \min\{\ms d_i(x_i^{m}(t_1+1),z_i^{m}(t_1+1)),s_{i+1}(x_i^{m}(t_1+1))\} =  \dfrac{y^{f^\text{in}}_i(t_1+1)}{\tilde{d}_{i+1,i+1}}.$

As for the cell $1$ and cell $I$, \eqref{eq:embedding-traffic} shows that the states only depend on cells $1,2$ and $I-1,I$ respectively, and the condition~\ref{ass:C-matrix-initial-final} in \Cref{ass:C-matrix} is obtained following the same analysis as above.
}

==> proof-linear-program-ks.tex <==
\subsection{On the Equivalence of \eqref{eq:saddle_point} and \eqref{eq:min-LP}}
\label{proof:prop-min-LP}
%For the proof, we shall make use of the following state transformation:
%\begin{equation*}
%\begin{bmatrix} z^m \\ z^r \end{bmatrix} = \begin{bmatrix} (\IR)^{-1} & 0 \\ 0 & I \end{bmatrix} \begin{bmatrix} x^m \\ x^r \end{bmatrix}
%\end{equation*}
%The dynamics \eqref{eq:cell_compact_dynamic} for this transformed variable is then:
%\begin{equation}
%\label{eq:transformed_flow}
%\begin{aligned}
%z^{m}(t+1) & = z^{m}(t) - f((\IR)z^{m}(t)) + (\IR)^{-1}u(t) \\
%z^{r}(t+1) &= z^{r}(t) - u(t) + \lambda
%\end{aligned}
%\end{equation}

%For given state trajectory for the ramps $x^r(t-L:t)$, input sequence $u(t-L:t-1)$, output sequence $y(t-L:t)$, and inflow rates $\lambda$ at the ramps, consider the relaxed problem of the minimization in \eqref{eq:saddle_point}, where $\hat{x}^{\circ,m}$ is the maximal element of $\mc X^m$ (cf. Lemma~\ref{lemm:maximal_element}):
%\begin{equation}
%	\begin{split} 
%		&	\underset{\substack{x(t-L:t+T),u(t:t+T-1)\\f(t-L:t+T-1)}}{\text{minimize}}%_{\substack{u(t:t+T-1) \in \mc U}} %_{\hat{u}(t:t+T-1)\in\mathcal{U}}
%			\sum_{s=t}^{t+T-1}l^\top  \, x(s)+ b^\top \, x(t+T) \\
%		\text{s.t.}\ &	x^m(s+1) = x^m(s) -(\IR)f(s) + u(s) %\label{eq:linear_program_mainstream_constraint}
%			%\text{s.t. }\, x^m_i(s+1) &= x^m_i(s) + \beta_{i-1}f_{i-1}(s) - f_{i}(s)+ u_{i}(s),
%			 ,\, s \in [t-L:t+T-1] \\ 
%			&x^r_i(s+1) = x^r_i(s) - u_{i}(s) + \lambda_i, \,i \in [I],\, s \in [t-L:t+T-1] \\
%			&f_i(s) \leq \min\{v_{i}x^m_{i}(s), \frac{w_{i+1}}{\beta_{i}} (\bar{x}_{i+1}-x^m_{i+1}(s))\}, \, i\in [I-1], \, s \in [t-L:t+T-1] \\
%			&f_{I}(s) \leq \min\{v_I x^m_I(s), \dfrac{v_iw_i}{v_i+w_i}\bar{x}\}, \, s \in [t-L:t+T-1] \\
%			&x(t-L) = \begin{bmatrix} \hat{x}^{\circ,m} \\ x^r(t-L) \end{bmatrix} \\
%			 &u_i(s)\in[0,\min\{x_i^r(s)+\lambda_i,\bar{u}_i\}]
%			 , \, i\in [I],\, s \in [t:t+T-1] 
%	\end{split}
%	\end{equation}
%The relaxation is to replace the flow equations in \eqref{eq:cell_dynamics} by inequalities \eqref{eq:lp-flow-equation1} and\eqref{eq:lp-flow-equation2}. Also,
%the second constraint in \eqref{eq:u-constraint} and the terminal constraint $x(t+T)\in\mc X_f$ is assumed to hold and removed in \eqref{eq:linear_program_saddle}.

	
%Then, we consider the transformed state $z^m(t)=(\IR)^{-1}x^m(t), z^r(t) = x^r(t)$ and
Consider the following linear program:
\ksmargin{why include $\Cm$ now?}
\begin{equation}	
	\begin{split}
			&\underset{\substack{z^m(t-L:t+T), \, x^r(t-L:t+T)\\ u(t:t+T-1), \, f(t-L:t+T-1)}}{\text{minimize}}%_{u(t:t+T-1)\in\mathcal{U}}&  \nonumber
			\sum_{s=t}^{t+T-1} l^{m\top}(\IR)z^{m}(s) + 
			 l^{r\top}x^{r}(s) \\ & \hspace{1.25in}+ b^{m\top} (\IR) z^{m}(t+T) +  b^{r\top} x^{r}(t+T)
			\\
			\text{s.t.}\ &z^{m}(s+1)\! =\! z^{m}(s) - f(s) + (\IR)^{-1}u(s), \, s\in [t-L:t+T-1] \\ 
			&x^r_i(s+1) = x^r_i(s) - u_{i}(s) + \lambda_i, \, i \in [I],\, s\in [t-L:t+T-1] \\
			&f_i(s) \leq  \min\left\{
			\begin{aligned}
				&v_{i-1}(z^m_{i}(s) - \beta_{i-1,i}z^m_{i-1}(s)) \\
				&\dfrac{w_{i+1}}{\beta_{i,i+1}}(\bar{x}_{i+1} - (z^m_{i+1}(s) - \beta_{i,i + 1}z^m_{i}(s)))\\
				&\kscomment{\Cm_i}
			\end{aligned}\right\}, \, i \in [I-1], s\in [t-L:t+T-1]\\
			&f_{I}(s) \leq \min\left\{
			\begin{aligned}
				&v_I(z^m_I (s)- \beta_{I-1,I}z^m_{I-1}(s)) \\
				&\Cm_I
			\end{aligned}
		\right\}, \, s\in [t-L:t+T-1]\\
		& z^m(t-L) =(\IR)^{-1}\hat{x}^{\circ,m} \\
%			&z(t-L) = \begin{bmatrix} 
%				(\IR)^{-1}\hat{x}^{\circ,m} \\ x^{r}(t-L)
%			\end{bmatrix} \\
					&u_i(s)\in[0,\min\{\bar{u}_i,x_i^{r}(t) +\lambda_i\}],\, i\in [I],\, s \in [t:t+T-1] 
					\end{split}
	\end{equation}
%	Note that the only operation transforming \eqref{eq:linear_program_saddle} to \eqref{eq:linear_program_transformed} is that we multiply $(\IR)^{-1}$ on both sides of the equation \eqref{eq:linear_program_mainstream_constraint}, which does not change the optimal solution because the feasible region and the objective function remain the same. Let $\hat{z}^{\circ,m} = (\IR)^{-1}\hat{x}^{\circ,m}$ and $V^*(\hat{z}^{\circ,m})$ denote the corresponding parameterized optimal objective value, we have $V^*(\hat{z}^{\circ,m})$ = $V^*(\hat{x}^{\circ,m})$. 

\ksmargin{need to discuss with ZL on how to write this compactly}
	Since $l^{m\top}(\IR)$ and $b^{m\top}(\IR)$ are nonnegative, we show by contradiction that for every optimal $u^*(t:t+T-1)$ to \eqref{eq:linear_program_transformed}, there exists an optimal solution $z^*(t-L:t+T)$ to \eqref{eq:linear_program_transformed} that is a state trajectory under \eqref{eq:transformed_flow}. Given any optimal $u^*(t:t+T-1)$, suppose every optimal solution is such that the constraints \eqref{eq:linear_program_transformed_flow1}, \eqref{eq:linear_program_transformed_flow2} are satisfied strictly for at least one time step and at least one cell. Let $\zopt(t-L:t+T)$ and $f^{\text{opt}}(t-L:t+T-1)$ denote the state values and flow rates of such an optimal solution. Let $\tilde{\phi}_{t-L}^s = \tilde{\phi}_{t-L}^s(\zopt(t-L), u^*(t-L:s-1)), s\in\{t-L,\ldots,t+T\}$. Without the loss of generality, we assume time $k$ is the first time there exists an strict inequality for \eqref{eq:linear_program_transformed_flow1}, \eqref{eq:linear_program_transformed_flow2}. When $s< k$, we have $\zopt(s) = \tilde{\phi}_{t-L}^s$. At time $k$, since there is an strict inequality, we have
\begin{multline*}
	\zoptm(k+1) = \zoptm(k) - f^{\text{opt}}(k) + (\IR)^{-1}\tilde{u}^*(k)
	\geq\tilde{\phi}_{t-L}^{k,m} - f((\IR)\tilde{\phi}_{t-L}^{k,m}) + (\IR)^{-1}\tilde{u}^*(k) = \tilde{\phi}_{t-L}^{k+1,m} 
	\end{multline*}
When $s>k$, from Lemma~\ref{lemm:monotone_z} we have
\begin{align*}
	\zoptm(s+1) = \zoptm(s) - f^{\text{opt}}(s) + (\IR)^{-1}\tilde{u}^*(s) 
	& \geq \zoptm(s) - f((\IR)\zoptm(s)) + (\IR)^{-1}\tilde{u}^*(s) \\
	& \geq\tilde{\phi}_{t-L}^{s,m}  - f((\IR)\tilde{\phi}_{t-L}^{s,m}) + (\IR)^{-1}\tilde{u}^*(s) = \tilde{\phi}_{t-L}^{s+1,m} 
\end{align*}
Therefore,
\begin{align*}
	V^*(\hat{z}^{\circ,m}) \geq \sum_{s=t}^{t+T-1}l^{m\top} (\IR)\tilde{\phi}_{t-L}^{s,m}+ l^{r\top} \tilde{\phi}_{t-L}^{s,r} 
	+b^{m\top}(\IR)\tilde{\phi}_{t-L}^{t+T,m}+ b^{r\top}\tilde{\phi}_{t-L}^{t+T,r}
\end{align*}
 which contradicts the fact that $\tilde{\phi}_{t-L}^{s}$ is not an optimal solution. Therefore, for any optimal $u^*(t:t+T-1)$ there exists an optimal solution $\zopt(s)= \tilde{\phi}_{t-L}^{s}, s\in\{t-L,\ldots,t+T\}$, which implies that $u^*(t:t+T-1)$ is also optimal for the minimization in \eqref{eq:saddle_point}.
 
 
\kscomment{
Let $\tilde{\phi}^t_0(z^{\circ},u(0:t-1))$ be the state $z(t)$ under \eqref{eq:transformed_flow} starting from initial condition $z^{\circ}$ and under control input $u(0:t-1)$. 
The following \emph{monotone} property proved in \cite{schmitt2020convexity} will be useful. 

\begin{lemma} \label{lemm:monotone_z}
	For any control sequence $u(0:t-1)$ and $z^{\circ,1} \leq z^{\circ,2}$, we have $\tilde{\phi}^t_0(z^{\circ,1},u(0:t-1)) \leq \tilde{\phi}^t_0(z^{\circ,2},u(0:t-1))$ %$\tilde{\phi}^t_0(z^{\circ,1},u(0:t-1)) \neq \tilde{\phi}^t_0(z^{\circ,2},u(0:t-1))$
	 for all $t \geq 0$.
\end{lemma}
}
 


==> proof-parameter-estimate-zl.tex <==
\subsection{Proof of Corollary~\ref{coro:parameter}}
\label{sec:parameter-estimate-proof}
By the proof of Theorem~\ref{theo:stability-boundedness}, the closed-loop system will enter $\mc X_f$ after finite time $K$ and the mainline state will stay uncongested. Then, the dynamics become
\begin{equation}\label{eq:cell-free-flow}
	\begin{aligned}
		x_i(t + 1) &= x_i(t) - v_ix_i(t) + u_i(t),\quad i=1 \\
		x_i(t+1) &= x_i(t) - \beta_{i-1}v_{i-1}x_{i-1}(t) + v_ix_i(t) + u_i(t), \\ &\hspace{2in}i\in[2:I] \\
	\end{aligned}
\end{equation}
Now we show that given $x_i(t),x_i(t-1),x_i(t-2) i\in[I]$ and $u_i(t),u_i(t-1), i\in[I]$, we can uniquely determine the value of $v$ and $\beta$. For $i=1$, the only unknown in \eqref{eq:cell-free-flow} is $v_1$ and thus $v_1$ can be uniquely determined. For $i=2$, we have
\begin{align*}
			x_2(t) &= x_2(t-1) + \beta_{1}v_{1}x_{1}(t-1) \\ &\quad- v_2x_2(t-1) + u_2(t-1) \\
			x_2(t-1) &= x_2(t-2) + \beta_1 v_{1} x_{1}(t-2) \\ &\quad - v_2 x_2(t-2) + u_2(t-2)
\end{align*}
The two unknowns are $\beta_1$ and $v_2$. Rearranging the equations gives
\begin{multline}\label{eq:parameter-matrix-form}
	\begin{bmatrix}
	 	v_1x_1(t-1) & -x_2(t-1) \\
	 	v_1x_1(t-2) & -x_2(t-2)
	\end{bmatrix}
	\begin{bmatrix}
		\beta_1 \\ v_2
	\end{bmatrix} \\ = 
\begin{bmatrix}
	x_2(t) - x_2(t-1) - u_2(t-1) \\ x_2(t-1) - x_2(t-2) - u_2(t-2)
\end{bmatrix}
\end{multline}
Then, it suffices to show that the $2\times 2$ matrix in \eqref{eq:parameter-matrix-form} has full rank. Since $x_1(t-1)/x_1(t-2) = 1 - v_2 + u_1(t) / x_1(t-2), x_2(t-1) / x_2(t-2) = 1 - v_2 + \beta_1v_1x_1(t-2)/x_2(t-2) +  u_2(t-2)/x_2(t-2)$, we have $x_1(t-1)/x_1(t-2) \neq x_2(t-1) / x_2(t-2)$ and the matrix has full rank. Therefore, $\beta_1$ and $v_2$ can be uniquely determined. By induction, given known $v_{i-1}$, we can always uniquely determine $\beta_{i-1}$ and $v_{i}$ for all $i\in[2:I]$. Therefore, $\ubar{v}(K+2) = \bar{v}(K+2) = v$ and $\ubar{\beta}(K+2) = \bar{\beta}(K+2)=\beta$.

==> proof-saddle-point-ks.tex <==
\subsection{Proof of Theorem~\ref{theo:existence_saddle}}
\label{proof:theo-existence-saddle-points} \ksmargin{I am not convinced about the uniqueness claim throughout the paper}
For every input sequence $\hat{u}(t:t+T-1)\in\mc U_{t-L:t}(T)$, the maximization problem in \eqref{eq:min-max}:
\begin{equation}\label{eq:saddle-point-max}
	\max_{(x^{\circ,m},z^{\circ,m}) \in\mc X^{\circ,m}_{t-L:t}}J(x^{\circ,m},z^{\circ,m},\hat{u}(t:t+T-1))
\end{equation}
admits an optimal solution $(x^{\circ,m,*},z^{\circ,m,*})$ which is the maximal/minimal element of $\mc X^{\circ,m}_{t-L:t}$. This is because every other $(x^{\circ,m},z^{\circ,m})\in \mc X^{\circ,m}_{t-L:t}$ satisfies that $x^{\circ,m}\leq x^{\circ,m,*}, z^{\circ,m}\geq z^{\circ,m,*}$, which implies that 
%\begin{equation*}
	$\Phi^{s,x,m}_{t-L}(x^{\circ,m},z^{\circ,m}, u(t-L:t-1), \hat{u}(t:s-1)) \leq 
	\Phi^{s,x,m}_{t-L}(x^{\circ,m,*},z^{\circ,m,*},u(t-L:t-1), \hat{u}(t:s-1))$ 
%\end{equation*}
for all $s\in[t-L:t+T]$ according to Lemma~\ref{lemm:embedding-system}. Since $l$ and $b$ are positive, this then implies $J(x^{\circ,m}, z^{\circ,m},\hat{u}(t:t+T-1)) \leq
	J(x^{\circ,m,*}, z^{\circ,m,*},\hat{u}(t:t+T-1))$.
 
Let $\hat{u}^*(t:t+T-1)$ be an optimal solution to the minimization problem in \eqref{eq:min-max}:
\begin{equation*}
	\min_{\hat{u}(t:t+T-1)\in\mc U_{t-L:t}(T)}J(x^{\circ,m,*}, z^{\circ,m,*} \hat{u}(t:t+T-1))
\end{equation*}
Therefore, $J^*=J(x^{\circ,m,*},z^{\circ,m,*}, \hat{u}^*(t:t+T-1))$. 
%
%The existence of solution is guaranteed since the objective is continuous and the set $\mc U$ is compact. Any optimal solution $\hat{u}^*(t:t+T-1)$ yields the same optimal value 
%\begin{equation*}
%	J_t(x^{\circ,m,*},\hat{u}^*(t:t+T-1)) = \min_{\hat{u}(t:t+T)\in\mc U}J_t(x^{\circ,m,*}, \hat{u}(t:t+T-1)) 
%\end{equation*}
%Also, 
Since $(x^{\circ,m,*},z^{\circ,m,*})$ is an optimal solution in \eqref{eq:saddle-point-max}, 
\begin{equation*}
	J(x^{\circ,m,*},z^{\circ,m,*},\hat{u}^*(t:t+T-1)) = \max_{(x^{\circ,m},z^{\circ,m}) \in\mc X^m}J(x^{\circ,m},z^{\circ,m},\hat{u}^*(t:t+T-1))
\end{equation*}
%Therefore, the pair of solutions $(x^{\circ,m,*},\hat{u}^*(t:t+T-1))$ satisfies \eqref{eq:saddle_point}. 



==> remarks-zl.tex <==
\subsection{Discussions}
\zl{
Some thoughts on the contribution of the controller
\begin{enumerate}
\item Mixed-monotonicity holds for quite general nonlinear systems \cite{yang2019sufficient}. This paper proposes a constructive way based on mixed-monotonicity to find saddle-point solutions of a min-max problem similar to the min-max certainty equivalence principle \cite{bernhard1995discrete}. Existence of saddle points is essential to show the certainty equivalence principle while it does not hold in general for nonlinear systems. Mixed-monotonicity could be useful to design certainty equivalent controllers for nonlinear systems.
\item To the best of my knowledge, mixed-monotonicity has not been used in the design of MPC control. \cite{heinlein2022robust} uses monotonicity to compute reachable sets and integrates them in the design of robust MPC.  The authors also claims that the next step is to extend the method to mixed-monotone systems.
\end{enumerate}
}

==> todo-ks.tex <==
\subsection{TODO}
In addition to the margins and comments in the text:
\begin{enumerate}
\item Should some $\prec$ be replaced with $\leq$ or vice-versa?
\item Modify abstract and introduction once comparison with open loop controller is well understood
\end{enumerate}
